Floyd-Warshall Reinforcement Learning: Learning from Past Experiences to Reach New Goals

Consider mutli-goal tasks that involve static environments and dynamic goals. Examples of such tasks, such as goal-directed navigation and pick-and-place in robotics, abound. Two types of Reinforcement Learning (RL) algorithms are used for such tasks: model-free or model-based. Each of these approaches has limitations. Model-free RL struggles to transfer learned information when the goal location changes, but achieves high asymptotic accuracy in single goal tasks. Model-based RL can transfer learned information to new goal locations by retaining the explicitly learned state-dynamics, but is limited by the fact that small errors in modelling these dynamics accumulate over long-term planning. In this work, we improve upon the limitations of model-free RL in multi-goal domains. We do this by adapting the Floyd-Warshall algorithm for RL and call the adaptation Floyd-Warshall RL (FWRL). The proposed algorithm learns a goal-conditioned action-value function by constraining the value of the optimal path between any two states to be greater than or equal to the value of paths via intermediary states. Experimentally, we show that FWRL is more sample-efficient and learns higher reward strategies in multi-goal tasks as compared to Q-learning, model-based RL and other relevant baselines in a tabular domain.

==> claims.tex <==
\subsection{Claims}
\begin{itemize} \item
Using FWRL is better than model-free learning like Q-learning in terms of generalizing to dynamic goals, static maps.
\item 
Using FWRL is better than model-based learning because of less accumulation over long term, hence more accurate value functions.
\item FWRL is better than Hindsight Experience Replay (HER) \cite{andrychowicz2016learning} because it is a parametric representation of hindsight.
\item FWRL is better than TDM~\cite{pong2018temporal} because it does not require the distance reward function.
\end{itemize}


==> future_work.tex <==

%\subsection{Future work}
%Items to improve the algorithm:
%\begin{itemize} \item
%\DONE{Justify the computational cost of constraint} The cost of going through the entire state space.
%How do you extend to a network? and large state spaces.
%\begin{enumerate}\item
%Observation 1: If there is only one goal, then the computation should not be any more than Q-learning.
%This can be accomplished by assuming that transitivity is satisfied till
%$\state_{t-1}$ and needs to be extend to only the next step. This sounds similar to the
% Floyd-Warshall dynamic programming update.
%However, this assumes that $\state_t$ is being visited for the first time.
%If the state $\state_t$ is being visited for the second time, the earlier
%value may be the shorter path for it.
%\end{enumerate}
%\item
%We need Q-value for exploration.
%\end{itemize}

